ProteinBench: A Holistic Evaluation of Protein Foundation Models

Recent years have witnessed a surge in the development of protein foundation models, significantly improving performance in protein prediction and generative tasks ranging from 3D structure prediction and protein design to conformational dynamics. However, the capabilities and limitations associated with these models remain poorly understood due to the absence of a unified evaluation framework. To fill this gap, we introduce ProteinBench, a holistic evaluation framework designed to enhance the transparency of protein foundation models. Our approach consists of three key components: (i) A taxonomic classification of tasks that broadly encompass the main challenges in the protein domain, based on the relationships between different protein modalities; (ii) A multi-metric evaluation approach that assesses performance across four key dimensions: quality, novelty, diversity, and robustness; and (iii) In-depth analyses from various user objectives, providing a holistic view of model performance. Our comprehensive evaluation of protein foundation models reveals several key findings that shed light on their current capabilities and limitations. To promote transparency and facilitate further research, we release the evaluation dataset, code, and a public leaderboard publicly for further analysis and a general modular toolkit. We intend for ProteinBench to be a living benchmark for establishing a standardized, in-depth evaluation framework for protein foundation models, driving their development and application while fostering collaboration within the field.

==> tables/conf_atlas_v2.tex <==
\begin{table}[t]\footnotesize
  \centering\setlength{\tabcolsep}{2pt}
  \caption{Performance on distribution prediction for the ATLAS test set. A total of 250 structures were sampled for each protein, and the median values across 82 proteins are reported. The \textbf{best} performance is highlighted in bold, and the \uline{second-best} is underlined. *These metrics require all-atom or backbone predictions; therefore, EigenFold and Str2Str do not have sufficient resolution for evaluation (indicated as ``N/A'').}

\resizebox{\textwidth}{!}{%

% \begin{tabular}{lllllllllllllllllll}
% \toprule
%  & \specialcell{Pairwise\\RMSD} & RMSF & \specialcell{Pairwise\\RMSD r} & \specialcell{Global\\RMSF r} & \specialcell{Per target\\RMSF r} & RMWD & \specialcell{MD PCA\\W2} & \specialcell{Joint\\PCA W2} & \specialcell{PC sim\\\> 0.5 \%} & \specialcell{Weak\\contacts J} & \specialcell{Transient\\contacts J} & \specialcell{Exposed \\residue J} & \specialcell{Exposed MI \\matrix rho} & \specialcell{CA-Break\\Rate \%} & \specialcell{CA-Clash\\Rate \%} & \specialcell{PepBond-Break\\Rate \%} & \specialcell{Secondary \\Structure \%} & \specialcell{Strand\\\%} \\
% \midrule
% \rowcolor{gray!15} MD (sample 250) & 2.76 & 1.63 & 0.96 & 0.97 & 0.99 & 0.71 & 0.76 & 0.7 & 93.9 & 0.9 & 0.8 & 0.93 & 0.56 & 0.0/0.0 & 0.1/0.0 & 3.4/3.4 & 59.6/58.4 & 18.5/18.3 \\
% EigenFold & 5.96 & 8.95 & -0.04 & 0.04 & 0.6 & 8.16 & 2.35 & 7.96 & 12.2 & 0.36 & 0.18 & nan & nan & 0.7/0.4 & 9.6/5.6 & nan/nan & 0.0/0.0 & 0.0/0.0 \\
% Str2Str-ODE (t=0.1) & 1.66 & 1.14 & 0.13 & 0.27 & 0.51 & 4.47 & 2.12 & 4.42 & 6.1 & 0.42 & 0.17 & 0.0 & -0.0 & 0.0/0.0 & 0.1/0.0 & 13.7/12.1 & 64.9/64.0 & 18.4/17.5 \\
% Str2Str-ODE (t=0.3) & 3.15 & 2.41 & 0.12 & 0.26 & 0.5 & 5.03 & 2.23 & 4.75 & 9.76 & 0.41 & 0.17 & 0.0 & -0.01 & 0.0/0.0 & 0.1/0.0 & 14.8/13.2 & 65.1/64.0 & 18.3/16.9 \\
% Str2Str-SDE (t=0.1) & 4.74 & 3.7 & 0.1 & 0.23 & 0.55 & 9.06 & 2.54 & 8.84 & 9.76 & 0.4 & 0.13 & 0.04 & 0.02 & 1.6/1.6 & 0.2/0.1 & 23.0/21.9 & 61.6/59.7 & 16.4/15.1 \\
% Str2Str-SDE (t=0.3) & 7.54 & 6.97 & 0.0 & 0.09 & 0.48 & 12.86 & 3.29 & 12.28 & 7.32 & 0.35 & 0.13 & 0.03 & 0.01 & 1.5/1.5 & 0.2/0.2 & 21.4/20.2 & 61.4/59.0 & 16.4/15.1 \\
% AlphaFlow-PDB & 2.58 & 1.2 & 0.27 & 0.46 & 0.81 & 2.96 & 1.66 & 2.6 & 37.8 & 0.44 & 0.33 & 0.42 & 0.18 & 0.0/0.0 & 0.2/0.1 & 6.6/6.7 & 62.6/62.0 & 19.3/18.9 \\
% AlphaFlow-MD & 2.88 & 1.63 & 0.53 & 0.66 & 0.85 & 2.68 & 1.53 & 2.28 & 39.02 & 0.57 & 0.38 & 0.5 & 0.24 & 0.0/0.0 & 0.2/0.0 & 21.7/22.2 & 61.9/61.5 & 19.1/18.6 \\
% ESMFlow-PDB & 3.0 & 1.68 & 0.14 & 0.27 & 0.71 & 4.2 & 1.77 & 3.54 & 28.05 & 0.42 & 0.29 & 0.41 & 0.16 & 0.0/0.0 & 0.6/0.2 & 5.4/5.1 & 62.0/61.7 & 18.3/17.7 \\
% ESMFlow-MD & 3.34 & 2.13 & 0.19 & 0.3 & 0.76 & 3.63 & 1.54 & 3.15 & 25.61 & 0.51 & 0.33 & 0.47 & 0.21 & 0.0/0.0 & 0.3/0.1 & 10.9/10.9 & 61.6/61.3 & 18.2/17.2 \\
% MSA-depth256 & 0.84 & 0.53 & 0.25 & 0.34 & 0.59 & 3.63 & 1.83 & 2.9 & 29.27 & 0.3 & 0.28 & 0.33 & 0.06 & 0.0/0.0 & 0.2/0.0 & 5.9/5.5 & 63.6/63.1 & 19.4/18.4 \\
% MSA-depth64 & 2.03 & 1.51 & 0.24 & 0.3 & 0.57 & 4.0 & 1.87 & 3.32 & 18.29 & 0.38 & 0.27 & 0.38 & 0.12 & 0.0/0.0 & 0.2/0.0 & 8.4/7.6 & 62.9/62.2 & 18.9/17.6 \\
% MSA-depth32 & 5.71 & 7.96 & 0.07 & 0.17 & 0.53 & 6.12 & 2.5 & 5.67 & 17.07 & 0.39 & 0.24 & 0.36 & 0.15 & 0.1/0.0 & 0.5/0.1 & 13.0/11.2 & 60.7/60.7 & 17.0/14.8 \\
% ConfDiff-ESM-PDB & 3.42 & 2.06 & 0.29 & 0.4 & 0.8 & 3.67 & 1.7 & 3.17 & 34.15 & 0.48 & 0.31 & 0.42 & 0.18 & 0.0/0.0 & 1.6/0.5 & 3.9/4.0 & 60.3/61.1 & 17.2/16.7 \\
% ConfDiff-Open-PDB & 2.9 & 1.43 & 0.38 & 0.51 & 0.82 & 2.97 & 1.57 & 2.51 & 34.15 & 0.47 & 0.34 & 0.43 & 0.18 & 0.0/0.0 & 0.9/0.5 & 5.7/5.6 & 61.7/61.4 & 19.0/18.1 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{Diversity}} & \multicolumn{3}{c}{\textbf{Flexibility: \textit{Pearson} $r$ on}} & \multicolumn{4}{c}{\textbf{Distributional accuracy}} \\
 \cmidrule(lr){2-3}  \cmidrule(lr){4-6} \cmidrule(lr){7-10}
 & \textbf{\specialcell{Pairwise\\RMSD}} & \textbf{*RMSF} & \specialcell{\textbf{Pairwise}\\\textbf{RMSD} ↑ } & \specialcell{*\textbf{Global}\\\textbf{RMSF} ↑ }  & \specialcell{*\textbf{Per target}\\\textbf{RMSF} ↑ } & \specialcell{*\textbf{RMWD} ↓} & \specialcell{\textbf{MD PCA}\\\textbf{W2} ↓} & \specialcell{\textbf{Joint}\\\textbf{PCA W2} ↓} & \specialcell{\textbf{PC sim}\\\textbf{$>$ 0.5 \%}↑ } \\
\midrule
\rowcolor{gray!15}
MD iid & 2.76 & 1.63 & 0.96 & 0.97 & 0.99 & 0.67 & 0.73 & 0.71 & 93.9 \\
\rowcolor{gray!15}
MD 2.5ns & 1.54 & 0.98 & 0.89 & 0.85 & 0.85 & 2.22 & 1.55 & 1.89 & 36.6 \\
EigenFold & 5.96 & 8.95 & -0.03 & 0.04 & 0.60 & 8.15 & 2.31 & 7.96 & 12.2 \\
MSA-depth256 & 0.83 & 0.53 & 0.25 & 0.34 & 0.59 & 3.60 & 1.79 & 2.91 & 29.3 \\
MSA-depth64 & 2.03 & 1.51 & 0.25 & 0.30 & 0.57 & 4.00 & 1.94 & 3.34 & 18.3 \\
MSA-depth32 & 5.70 & 7.96 & 0.08 & 0.17 & 0.53 & 6.09 & 2.56 & 5.70 & 17.1 \\
Str2Str-ODE ($T_\text{max}=0.1$) & 1.66 & 1.14 & 0.13 & 0.27 & 0.51 & 4.49 & 2.14 & 4.39 & 6.1 \\
Str2Str-ODE ($T_\text{max}=0.3$) & 3.15 & 2.41 & 0.13 & 0.26 & 0.50 & 5.05 & 2.19 & 4.80 & 9.8 \\
Str2Str-SDE ($T_\text{max}=0.1$) & 4.74 & 3.70 & 0.11 & 0.23 & 0.55 & 9.06 & 2.54 & 8.82 & 9.8 \\
Str2Str-SDE ($T_\text{max}=0.3$) & 7.54 & 6.97 & 0.01 & 0.09 & 0.48 & 12.87 & 3.24 & 12.28 & 7.3 \\
AlphaFlow-PDB & 2.58 & 1.20 & 0.27 & 0.46 & 0.81 & 2.97 & 1.61 & 2.61 & 37.8 \\
AlphaFlow-MD & 2.87 & 1.63 & 0.53 & 0.66 & 0.85 & 2.64 & 1.55 & 2.29 & 39.0 \\
ESMFlow-PDB & 2.99 & 1.68 & 0.14 & 0.27 & 0.71 & 4.15 & 1.87 & 3.61 & 28.0 \\
ESMFlow-MD & 3.33 & 2.13 & 0.19 & 0.30 & 0.76 & 3.61 & 1.66 & 3.25 & 25.6 \\
ConfDiff-AF2-clsfree_0.8 & 3.68 & 2.12 & 0.39 & 0.54 & 0.83 & 2.91 & 1.54 & 2.46 & 46.3 \\
ConfDiff-AF2-PDB & 2.89 & 1.43 & 0.38 & 0.51 & 0.82 & 2.96 & 1.59 & 2.46 & 34.1 \\
ConfDiff-AF2-MD & 3.43 & 2.21 & 0.59 & 0.67 & 0.85 & 2.75 & 1.41 & 2.27 & 35.4 \\
ConfDiff-ESM-clsfree_0.8 & 4.04 & 2.84 & 0.31 & 0.43 & 0.82 & 3.78 & 1.73 & 3.07 & 37.8 \\
ConfDiff-ESM-PDB & 3.42 & 2.06 & 0.29 & 0.40 & 0.80 & 3.62 & 1.68 & 3.13 & 34.1 \\
ConfDiff-ESM-MD & 3.90 & 2.79 & 0.35 & 0.48 & 0.82 & 3.62 & 1.73 & 3.00 & 37.8 \\
\bottomrule
 & \multicolumn{4}{c}{\textbf{Ensemble observables}} & \multicolumn{3}{c}{\textbf{Quality}}  \\
  \cmidrule(lr){2-5}  \cmidrule(lr){6-8}
 & \specialcell{\textbf{Weak}\\\textbf{contacts $J$} ↑} & \specialcell{\textbf{Transient}\\\textbf{contacts $J$}↑} & \specialcell{*\textbf{Exposed} \\\textbf{residue $J$} ↑} & \specialcell{*\textbf{Exposed MI} \\\textbf{matrix $\rho$} ↑} & \specialcell{\textbf{CA break}\\\textbf{\%} ↓} & \specialcell{\textbf{CA clash}\\\textbf{\%} ↓} & \specialcell{\textbf{PepBond}\\\textbf{break \%} ↓} &  &   \\
\midrule
\rowcolor{gray!15} 
MD iid & 2.76 & 1.63 & 0.96 & 0.97 & 0.99 & 0.67 & 0.73 & 0.71 & 93.9 \\
\rowcolor{gray!15}
MD 2.5ns & 0.62 & 0.45 & 0.64 & 0.25 & 0.0 & 0.0 & 3.4 \\
EigenFold & 0.36 & 0.19 & nan & nan & 5.6 & 0.4 & nan \\
MSA-depth256 & 0.30 & 0.29 & 0.36 & 0.06 & 0.0 & 0.0 & 5.5 \\
MSA-depth64 & 0.38 & 0.28 & 0.40 & 0.16 & 0.0 & 0.0 & 7.6 \\
MSA-depth32 & 0.40 & 0.24 & 0.40 & 0.19 & 0.1 & 0.0 & 11.2 \\
Str2Str-ODE ($T_\text{max}=0.1$) & 0.42 & 0.18 & 0.50 & 0.17 & 0.0 & 0.0 & 12.1 \\
Str2Str-ODE ($T_\text{max}=0.3$) & 0.42 & 0.17 & 0.53 & 0.25 & 0.0 & 0.0 & 13.2 \\
Str2Str-SDE ($T_\text{max}=0.1$) & 0.40 & 0.13 & 0.52 & 0.23 & 0.1 & 1.6 & 21.9 \\
Str2Str-SDE ($T_\text{max}=0.3$) & 0.36 & 0.13 & 0.52 & 0.20 & 0.2 & 1.5 & 20.2 \\
AlphaFlow-PDB & 0.45 & 0.36 & 0.50 & 0.25 & 0.1 & 0.0 & 6.7 \\
AlphaFlow-MD & 0.62 & 0.41 & 0.69 & 0.35 & 0.0 & 0.0 & 22.2 \\
ESMFlow-PDB & 0.42 & 0.30 & 0.46 & 0.21 & 0.2 & 0.0 & 5.1 \\
ESMFlow-MD & 0.55 & 0.34 & 0.57 & 0.29 & 0.1 & 0.0 & 10.9 \\
ConfDiff-AF2-clsfree_0.8 & 0.58 & 0.36 & 0.60 & 0.28 & 0.8 & 0.0 & 5.7 \\
ConfDiff-AF2-PDB & 0.50 & 0.36 & 0.54 & 0.25 & 0.5 & 0.0 & 5.6 \\
ConfDiff-AF2-MD & 0.63 & 0.39 & 0.65 & 0.33 & 0.5 & 0.0 & 6.5 \\
ConfDiff-ESM-clsfree_0.8 & 0.57 & 0.34 & 0.59 & 0.23 & 0.9 & 0.0 & 4.3 \\
ConfDiff-ESM-PDB & 0.50 & 0.33 & 0.50 & 0.24 & 0.5 & 0.0 & 4.0 \\
ConfDiff-ESM-MD & 0.61 & 0.36 & 0.61 & 0.31 & 0.4 & 0.0 & 4.3 \\
\bottomrule
\end{tabular}
}%
\label{tab:conf_atlas_v2}%
\end{table}%j
